Fast Langevin based algorithm for MCMC in high dimensions

We introduce new Gaussian proposals to improve the efficiency of the standard Hastings-Metropolis algorithm in Markov chain Monte Carlo (MCMC) methods, used for the sampling from a target distribution in large dimension $d$. The improved complexity is $\mathcal{O}(d^{1/5})$ compared to the complexity $\mathcal{O}(d^{1/3})$ of the standard approach. We prove an asymptotic diffusion limit theorem and show that the relative efficiency of the algorithm can be characterised by its overall acceptance rate (with asymptotical value 0.704), independently of the target distribution. Numerical experiments confirm our theoretical findings.

==> technical_results.tex <==
\section{Postponed proofs}
\label{sec:app_tech_proof}
\subsection{Proof of Lemma~\ref{propo:convergence_gaussian_proposal}}
\label{subsec:lemme_convergence_gaussian_proposal}
%\begin{proof}[Proof of Lemma~\ref{propo:convergence_gaussian_proposal}]
    By Assumption \ref{hyp:Gaussian_Markov_kernel}-\ref{hyp:density_convergence}, $\pi$ and $q$ are positive and continuous. It follows from  \cite[Lemma
    1.2]{mengersen:tweedie:1996} that  $P$ is $\Leb^d$-irreducible aperiodic, where $\Leb^d$ is the
    Lebesgue measure on $\IR^d$. In addition, all compact set $\smallSet$ such that $\Leb^d(\smallSet)
    >0$ are small for $P$. Now by \cite[Theorem 15.0.1]{meyn:tweedie:2009}, we just need
    to check the drift condition \eqref{eq:drift_condition}. But by a simple calculation, using $\alpha(x,y) \leq 1$ for all $x,y \in \rset^d$, and the Cauchy-Schwarz inequality, we get
\begin{align*}
  PV(\varx) %&\leq 1 + \norm{\mu(\varx)}^2 \int_{\IR^d} \alpha(\varx,\vary) q(\varx,\vary)
%  \rmd
%  \vary
%  + (2 \uppi)^{-d/2} \int_{\IR^d} \norm{S(\varx)
%    \GaussianRV}^2
%  \exp(-\norm{\GaussianRV}^2/2) \rmd \GaussianRV \\
%&  + 2(2 \uppi)^{-d/2} \norm{\mu(\varx)} \int_{\IR^d} \norm{S(\varx) \GaussianRV}
%  \exp(-\norm{\GaussianRV}^2/2)\rmd \GaussianRV + \norm{x}^2 \int_{\IR^d} (1-\alpha(\varx,\vary)) q(\varx,\vary) \rmd \vary\\
  & \leq 1 +  \norm{\varx}^2
  + (\norm{\mu(\varx)}^2-\norm{\varx}^2) \int_{\IR^d} \alpha(\varx,\vary) q(\varx,\vary) \rmd \vary \\
  & + (2 \uppi)^{-d/2} (2\norm{\mu(\varx)} \norm{S(\varx)} + \norm{S(\varx)}^2)\int_{\IR^d} \max(\norm{
    \GaussianRV}^2 , 1)
  \rme^{-\norm{\GaussianRV}^2/2} \rmd \GaussianRV \eqsp.
  \end{align*}
  By \eqref{eq:hyp:gaussian_prop_mu}, $ \limsup_{\norm{x} \to
    \plusinfty}(2\norm{\mu(\varx)} \norm{S(\varx)} +
  \norm{S(\varx)}^2)\norm{x}^{-2} = 0  $. Therefore, using again
  the first inequality of \eqref{eq:hyp:gaussian_prop_mu} and  Assumption \ref{hyp:ratio_convergence_bO}:
\begin{equation*}
\limsup_{\norm{\varx} \to \plusinfty} PV(\varx) /V(\varx) \leq 1-(1-\tau^2) \liminf _{\norm{\varx} \to \plusinfty} \int_{\IR^d} \alpha(\varx,\vary) q(\varx,\vary) \rmd
\vary < 1 \eqsp.
% \leq  1-(1-\tau^2)\kappa \eqsp,
\end{equation*}
%This concludes the proof upon noting $1 - (1-\tau^2) \kappa < 1$.
 This concludes the proof  of Lemma~\ref{propo:convergence_gaussian_proposal}.\qed   
%\end{proof} 
\subsection{Proof of Theorem~\ref{theo:non_geo_erg_Gaussian_MH}}
%\begin{proof}[Proof of Theorem~\ref{theo:non_geo_erg_Gaussian_MH}]
\label{subsec:proof_theo_non_geo}
We prove this result by contradiction. The strategy of the proof is the following: first, under our
assumptions, most of the proposed moves by the algorithm has a norm which is
greater than the current point. However,  if $P$ is geometrically ergodic, then it implies a  upper bound on the rejection
probability of the algorithm by some constant strictly smaller than $1$. But combining these facts, we can exhibit a sequence of point
$\{ x_n , n \in \nset \}$, such that $\lim_{n \to \plusinfty} \pi(x_n) =
\plusinfty$. Since we assume that $\pi$ is bounded, we have our contradiction.

If $P$ is geometrically ergodic, then by
\cite[Theorem 5.1]{roberts:tweedie:1996}, there exists $\eta >0$ such that for almost every $x \in
\rset^d$,
\begin{equation}
  \label{eq:bound_rejection_proba}
\int_{\rset^d} \alpha(x,y) q(x,y) \rmd y \geq  \eta \eqsp,
\end{equation}
and let $M \geq 0$ such that
\begin{equation}
\label{eq:def_M_non_geo}
\mathbb{P}\left[ \norm{\xi} \geq M \right] \leq \eta /2 \eqsp,
\end{equation}
where $\xi$ is a standard $d$-dimensional Gaussian random variable. By \eqref{eq:assum_theo_non_geo}, there
exists $R_\epsilon , \delta > 0$ such that
\begin{equation}
  \label{def_R_epsilon_non_geo}
\inf_{\{ \norm{x} \geq R_\epsilon \}} \norm{S(x)^{-1} \mu(x)}\norm{x}^{-1} \geq
\epsilon^{-1} + \delta \ \text{ and } \inf_{\{ \norm{x} \geq R_\epsilon \}} \inf_{\norm{y}
    = 1} \norm{S(x)y} \geq \epsilon \eqsp.
\end{equation}
Note that we can assume $R_\epsilon$ is large enough so that
\begin{equation}
  \label{eq:condition_R_epsi}
\epsilon \delta R _\epsilon
\geq M   \eqsp.
\end{equation}
Now define for $x \in \rset^d$, $\norm{x} \geq R_\epsilon$
\begin{equation}
  \label{eq:defBx}
B(x) = \left\lbrace y \in \rset^d \ |  \   \norm{S(x)^{-1} (y - \mu(x) )} \leq M
\right\rbrace \eqsp.
\end{equation}
Note if $y \in B(x)$, we have by definition and the triangle inequality $\norm{S(x)^{-1}y } \geq \norm{S(x)^{-1}
  \mu(x)} -M$. Therefore by   \eqref{def_R_epsilon_non_geo} and \eqref{eq:condition_R_epsi}
\begin{equation}
  \label{eq:norm_propo_greater}
\norm{y} = \norm{S(x) S(x)^{-1} y } \geq \epsilon \norm{S(x)^{-1} y} \geq
\epsilon(\epsilon^{-1}+\delta)\norm{x} -M \geq \norm{x} \eqsp.
  \end{equation}
  We then show that this inequality implies
\begin{equation}
  \label{eq:ratio_q_zeros}
  \liminf_{\norm{x} \to \plusinfty} \inf_{y \in
  B(x)} \frac{q(y,x)}{q(x,y)} = 0 \eqsp.
\end{equation}
First, it is straightforward by \eqref{eq:defBx}, that the denominator is uniformly
bounded from $0$. As for the numerator, first we can notice by
\eqref{def_R_epsilon_non_geo}-\eqref{eq:norm_propo_greater}, we have $\norm{y} \geq R_\epsilon$ and for all $z \in
\rset^d$, $\norm{S(y)z} \geq \epsilon \norm{z}$, which implies for all $z \in \rset^d$,
$\epsilon^{-1}\norm{z} \geq \norm{S(y)^{-1} z}$. Using this result, the triangle
inequality and \eqref{def_R_epsilon_non_geo}-\eqref{eq:norm_propo_greater} again, we get
\begin{align*}
q(y,x) &= (2\uppi)^{-d/2}\exp \left(-\norm{S(y)^{-1} (x-\mu(y))}^2 - \log( \abs{S(y) (S(y))^T} ) \right) \\
& \leq  (2\uppi)^{-d/2}\exp \left(-(\norm{S(y)^{-1}\mu(y)} - \norm{S(y)^{-1} x})^2 - \log(
  \abs{S(y) (S(y))^T} ) \right) \\
& \leq   (2\uppi)^{-d/2}\exp \left(-((\epsilon^{-1} + \delta)\norm{y} - \epsilon^{-1}\norm{y})^2 - \log(
  \abs{S(y) (S(y))^T} ) \right) \\
& \leq   (2\uppi)^{-d/2}\exp \left(-\delta^2 \norm{y}^2 - \log(
  \abs{S(y) (S(y))^T} ) \right) \eqsp.
  \end{align*}
  Using this inequality and \eqref{eq:assum_theo_non_geo2} imply $\lim_{\norm{x} \to
    \plusinfty} \inf_{y \in B(x)} q(y,x) =0$ and then
  \eqref{eq:ratio_q_zeros}. Therefore there exists $R_q \geq 0$ such that for all $x \in
  \rset^d$, $\norm{x} \geq R_q$
  \begin{equation}
\label{eq:def_Rq}
\inf_{y \in B(x)} \frac{q(y,x)}{q(x,y)}  \leq \eta/4 \eqsp.
    \end{equation}
    Now we are able to build the sequence $\{ x_n , n \in \nset\}$ such that for all $n
    \in \nset$, $\norm{x_{n+1}} \geq \max( R_\epsilon, R_q)$ and $\lim_{n \to \plusinfty} \pi(x_n) =
    \plusinfty$. Indeed let $x_0 \in \rset^d$ such that $\norm{x_0} \geq \max( R_\epsilon,
    R_q)$. Assume, we have built the sequence up to the $n$th term and such that for all
    $k=0, \dots, n-1$, $\norm{x_{k+1}} \geq \max( R_\epsilon, R_q)$ and $\pi(x_{k+1}) \geq
    (3/2) \pi(x_k)$. Now we choose $x_{n+1}$ depending
    on $x_n$, satisfying $\pi(x_{n+1}) \geq (3/2) \pi(x_n)$ and $ \norm{x_{n+1}} \geq \max( R_\epsilon, R_q)$. Since
    $\norm{x_n} \geq  \max( R_\epsilon, R_q)$, by
    \eqref{eq:bound_rejection_proba}-\eqref{eq:def_M_non_geo} and \eqref{eq:def_Rq}
  \begin{align*}
\eta &\leq \int_{\rset^d} \alpha(x_n,y) q(x_n,y) \rmd y  \leq \eta/2 + \int_{B(x_n)}
\min \left(1, \frac{\pi(y)q(y,x_n)}{\pi(x_n) q(x_n,y)} \right)  q(x_n,y) \rmd y \\
& \leq \eta/2 + ( \eta/4)\int_{B(x_n)}\frac{\pi(y)}{\pi(x_n)} q(x_n,y) \rmd y \eqsp.
    \end{align*}
    This inequality implies that $\int_{B(x_n)}\frac{\pi(y)}{\pi(x_n)} q(x_n,y) \rmd y  \geq
    2$ and therefore there exists $x_{n+1} \in B(x_n)$ such that $\pi(x_{n+1})
    \geq (3/2)\pi(x_n)$, and since $x_{n+1} \in B(x_n)$ by \eqref{eq:norm_propo_greater},
    $\norm{x_{n+1}} \geq  \max( R_\epsilon, R_q)$. Therefore, we have a sequence $\{x_n ,
    n \in \nset \}$ such that for all $n \in \nset$, $ \pi(x_{n+1}) \geq (3/2)\pi(x_n)$. Since
    by assumption $\pi(x_0) >0$, we get $\lim_{n \to \plusinfty} \pi(x_n) = \plusinfty$,
    which contradicts the assumption that $\pi$ is bounded.
  %\end{proof}
This concludes the proof  of Theorem~\ref{theo:non_geo_erg_Gaussian_MH}.\qed  


\subsection{Technical results}
\begin{lemma}
\label{lem:fun_positive}
The following functions on $\rset^*$ can be extended to continuous and positive functions on $\rset$:
\begin{enumerate}[(a)]
\item
\label{lem:fun_positive_1}
$\Psi_1 : t \mapsto \{ \rme^{t}-1 - (1/3)t^2 \}/t $.
\item\label{lem:fun_positive_2}
$\Psi_2 : t \mapsto \{\rme^{t}-1 + (1/3)(\rme^{-t^2}-1)\}/t $.
\end{enumerate}
\end{lemma}

\begin{proof}
It is straightforward that $\Psi_1$ and $\Psi_2$ can be extended to a continuous function,
setting $\Psi_1(0) = 1$ and $\Psi_2(0)=1$. Moreover, since for all $t <0$, $\rme^{t} < 1$,
these two functions are positive on $\rset^*_-$. Now, we study the sign of each one on
$\rset^*_+$.
For all $u >0$, $\rme^{u} \geq u $. Integrating this inequality from $0$ to $t >0$, we
have $\rme^{t} -1 \geq (1/2) t^2$, which implies that $\Psi_1$ is positive on
$\rset^*_+$. This latter relation also implies that $\Psi_2$ is positive on $\rset^*_+$
since for all $t >0$, $t \in \rset$, $1-\rme^{t^2} \leq t^2$.
\end{proof}

\begin{lemma}
\label{lem:fun_positive_ergodicity1}
The function $\Psi$ defined on $\coint{3, \plusinfty}$ by
\begin{multline*}
\Psi(t) =   1-\defSet{1-\frac{5}{3(t-1)}}^t  \\ - (3/8)t(t-1) \defSet{
1-\bracket{1-\frac{5}{3(t-1)}}^2 }^2 \defSet{1-\frac{5}{3(t-1)} }^{t-2} \eqsp,
\end{multline*}
is positive on $\coint{3, \plusinfty}$.
\end{lemma}

\begin{proof}
First  we can write
\[
\Psi(t) = 1-\defSet{1-\frac{5}{3(t-1)}}^t   - \frac{25t}{24(t-1)} \defSet{
2-\frac{5}{3(t-1)} }^2 \defSet{1-\frac{5}{3(t-1)} }^{t-2} \eqsp.
\]
Since the functions
\begin{equation*}
 t \mapsto \defSet{1-\frac{5}{3(t-1)}}^t \eqsp, \quad
 t \mapsto \frac{25t}{24(t-1)} \defSet{
2-\frac{5}{3(t-1)} }^2 \defSet{1-\frac{5}{3(t-1)} }^{t-2}
\end{equation*}
are increasing on $\coint{3,\plusinfty}$, we can conclude that
\[
\inf_{ t \in \coint{5, \plusinfty} }\Psi(t) \geq \lim_{ t \to \plusinfty} \Psi(t) = 1- \frac{31 \rme^{-5/3}}{6} >0 \eqsp.
\]
\end{proof}

\begin{lemma}
\label{lem:fun_positive_ergodicity2}
For all $t,h,\lambda >0$, define the functions $\varrho$, $\varsigma$ and $\Xi$ by:
\begin{align*}
\varrho(t) &= (\rme^{-t} - 1) + (2/3)(\rme^{-t^2}- 1) \eqsp, \\
\varsigma(t) &= (\rme^{-2 t}-1) +(1/3)(\rme^{-4 t^2}-1)  \eqsp, \\
\Xi(h, \lambda)  &= \lambda \bracket{ 1 - (\varrho(h \lambda)+1)^2  +
  \varsigma(h \lambda)^{-1}\bracket{4\varrho(h \lambda)^2 + 4 \varrho(h \lambda)^3 +
    \varrho(h \lambda)^4} }\eqsp.
\end{align*}
Then for all $h,\lambda >0$, $\Xi(h, \lambda) >0$.
\end{lemma}

\begin{proof}
We just need to check that the function $\psi$ defined by for all $t >0$
\[
\psi(t) = 1 - (\varrho(t)+1)^2  +
  \varsigma(t)^{-1}\bracket{4\varrho(t)^2 + 4 \varrho(t)^3 +
    \varrho(t)^4} \eqsp,
\]
is positive on $\rset_+^*$. But since for all $t >0$, $\varsigma(t) > \varrho(t) +\varrho(t)^2/2$,
\[
\psi(t) > 1 - (\varrho(t)+1)^2  +
  (\varrho(t) +\varrho(t)^2/2)^{-1}\bracket{4\varrho(t)^2 + 4 \varrho(t)^3 +
    \varrho(t)^4} =0 \eqsp.
\]
This concludes the proof.
\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "MCMC_final1"
%%% End: 


==> technical_results1.tex <==
\section{Postponed proofs}
\label{sec:app_tech_proof}
\subsection{Proof of Lemma~\ref{propo:convergence_gaussian_proposal}}
\label{subsec:lemme_convergence_gaussian_proposal}
%\begin{proof}[Proof of Lemma~\ref{propo:convergence_gaussian_proposal}]
    By Assumption \ref{hyp:Gaussian_Markov_kernel}-\ref{hyp:density_convergence}, $\pi$ and $q$ are positive and continuous. It follows from  \cite[Lemma
    1.2]{mengersen:tweedie:1996} that  $P$ is $\Leb^d$-irreducible aperiodic, where $\Leb^d$ is the
    Lebesgue measure on $\IR^d$. In addition, all compact set $\smallSet$ such that $\Leb^d(\smallSet)
    >0$ are small for $P$. Now by \cite[Theorem 15.0.1]{meyn:tweedie:2009}, we just need
    to check the drift condition \eqref{eq:drift_condition}. But by a simple calculation, using $\alpha(x,y) \leq 1$ for all $x,y \in \rset^d$, and the Cauchy-Schwarz inequality, we get
\begin{align*}
  PV(\varx) %&\leq 1 + \norm{\mu(\varx)}^2 \int_{\IR^d} \alpha(\varx,\vary) q(\varx,\vary)
%  \rmd
%  \vary
%  + (2 \uppi)^{-d/2} \int_{\IR^d} \norm{S(\varx)
%    \GaussianRV}^2
%  \exp(-\norm{\GaussianRV}^2/2) \rmd \GaussianRV \\
%&  + 2(2 \uppi)^{-d/2} \norm{\mu(\varx)} \int_{\IR^d} \norm{S(\varx) \GaussianRV}
%  \exp(-\norm{\GaussianRV}^2/2)\rmd \GaussianRV + \norm{x}^2 \int_{\IR^d} (1-\alpha(\varx,\vary)) q(\varx,\vary) \rmd \vary\\
  & \leq 1 +  \norm{\varx}^2
  + (\norm{\mu(\varx)}^2-\norm{\varx}^2) \int_{\IR^d} \alpha(\varx,\vary) q(\varx,\vary) \rmd \vary \\
  & + (2 \uppi)^{-d/2} (2\norm{\mu(\varx)} \norm{S(\varx)} + \norm{S(\varx)}^2)\int_{\IR^d} \max(\norm{
    \GaussianRV}^2 , 1)
  \rme^{-\norm{\GaussianRV}^2/2} \rmd \GaussianRV \eqsp.
  \end{align*}
  By \eqref{eq:hyp:gaussian_prop_mu}, $ \limsup_{\norm{x} \to
    \plusinfty}(2\norm{\mu(\varx)} \norm{S(\varx)} +
  \norm{S(\varx)}^2)\norm{x}^{-2} = 0  $. Therefore, using again
  the first inequality of \eqref{eq:hyp:gaussian_prop_mu} and  Assumption \ref{hyp:ratio_convergence_bO}:
\begin{equation*}
\limsup_{\norm{\varx} \to \plusinfty} PV(\varx) /V(\varx) \leq 1-(1-\tau^2) \liminf _{\norm{\varx} \to \plusinfty} \int_{\IR^d} \alpha(\varx,\vary) q(\varx,\vary) \rmd
\vary < 1 \eqsp.
% \leq  1-(1-\tau^2)\kappa \eqsp,
\end{equation*}
%This concludes the proof upon noting $1 - (1-\tau^2) \kappa < 1$.
 This concludes the proof  of Lemma~\ref{propo:convergence_gaussian_proposal}.\qed
%\end{proof}
\subsection{Proof of Theorem~\ref{theo:non_geo_erg_Gaussian_MH}}
%\begin{proof}[Proof of Theorem~\ref{theo:non_geo_erg_Gaussian_MH}]
\label{subsec:proof_theo_non_geo}
We prove this result by contradiction. The strategy of the proof is the following: first, under our
assumptions, most of the proposed moves by the algorithm has a norm which is
greater than the current point. However,  if $P$ is geometrically ergodic, then it implies a  upper bound on the rejection
probability of the algorithm by some constant strictly smaller than $1$. But combining these facts, we can exhibit a sequence of point
$\{ x_n , n \in \nset \}$, such that $\lim_{n \to \plusinfty} \pi(x_n) =
\plusinfty$. Since we assume that $\pi$ is bounded, we have our contradiction.

If $P$ is geometrically ergodic, then by
\cite[Theorem 5.1]{roberts:tweedie:1996}, there exists $\eta >0$ such that for almost every $x \in
\rset^d$,
\begin{equation}
  \label{eq:bound_rejection_proba}
\int_{\rset^d} \alpha(x,y) q(x,y) \rmd y \geq  \eta \eqsp,
\end{equation}
and let $M \geq 0$ such that
\begin{equation}
\label{eq:def_M_non_geo}
\mathbb{P}\left[ \norm{\xi} \geq M \right] \leq \eta /2 \eqsp,
\end{equation}
where $\xi$ is a standard $d$-dimensional Gaussian random variable. 
\moda{By \eqref{eq:assum_theo_non_geo}, there
exist $R_\epsilon , \delta > 0$ such that
\begin{align}
  \label{def_R_epsilon_non_geo1}
\inf_{\{ \norm{x} \geq R_\epsilon \}} \norm{S(x)^{-1} \mu(x)}\norm{x}^{-1} &\geq
\epsilon^{-1} + \delta \ \\
  \label{def_R_epsilon_non_geo2}
 \inf_{\{ \norm{x} \geq R_\epsilon \}} \inf_{\norm{y}
    = 1} \norm{S(x)y} &\geq \epsilon (1+ \delta\epsilon/2)^{-1} \eqsp.
\end{align}
Note that we can assume $R_\epsilon$ is large enough so that
\begin{equation}
  \label{eq:condition_R_epsi}
\epsilon \delta R _\epsilon/2
\geq M   \eqsp.
\end{equation}
Now define for $x \in \rset^d$, $\norm{x} \geq R_\epsilon$
\begin{equation}
  \label{eq:defBx}
B(x) = \left\lbrace y \in \rset^d \ |  \   \norm{S(x)^{-1} (y - \mu(x) )} \leq M
\right\rbrace \eqsp.
\end{equation}
Note if $y \in B(x)$, we have by definition and the triangle inequality $\norm{S(x)^{-1}y } \geq \norm{S(x)^{-1}
  \mu(x)} -M$. Therefore by   \eqref{def_R_epsilon_non_geo1}-\eqref{def_R_epsilon_non_geo2} and \eqref{eq:condition_R_epsi}
\begin{multline}
  \label{eq:norm_propo_greater}
\norm{y} = \norm{S(x) S(x)^{-1} y } \geq \epsilon (1+ \delta\epsilon/2)^{-1} \norm{S(x)^{-1} y} \\
\geq
\epsilon (1+ \delta\epsilon/2)^{-1} \defEns{(\epsilon^{-1}+\delta)\norm{x} -M} \geq \norm{x} \eqsp.
  \end{multline}
  We then show that this inequality implies
\begin{equation}
  \label{eq:ratio_q_zeros}
  \liminf_{\norm{x} \to \plusinfty} \inf_{y \in
  B(x)} \frac{q(y,x)}{q(x,y)} = 0 \eqsp.
\end{equation}
First, it is straightforward by \eqref{eq:defBx}, that $\abs{S(x)}q(x,y)$ is uniformly
bounded from $0$, and it suffices to consider $\abs{S(x)}q(y,x)$. By
\eqref{def_R_epsilon_non_geo2}-\eqref{eq:norm_propo_greater}, we have $\norm{y} \geq R_\epsilon$ and for all $z \in
\rset^d$, $\norm{S(y)z} \geq \epsilon (1+ \delta\epsilon/2)^{-1} \norm{z}$, which implies for all $z \in \rset^d$,
$\epsilon^{-1}(1+ \delta\epsilon/2)\norm{z} \geq \norm{S(y)^{-1} z}$. Using this result, the triangle
inequality and \eqref{def_R_epsilon_non_geo1}-\eqref{def_R_epsilon_non_geo2}-\eqref{eq:norm_propo_greater}, we get
\begin{align*}
q(y,x) &= (2\uppi)^{-d/2}\exp \defEns{-(1/2) \norm{S(y)^{-1} (x-\mu(y))}^2 - \log( \abs{S(y) } ) } \\
& \leq  (2\uppi)^{-d/2}\exp \defEns{-(1/2)\bracket{\norm{S(y)^{-1}\mu(y)} - \norm{S(y)^{-1} x}}^2 - \log(
  \abs{S(y) } ) } \\
% & \leq   (2\uppi)^{-d/2}\exp \defEns{-(1/2)((\epsilon^{-1} + \delta)\norm{y} - \epsilon^{-1}(1+ \delta\epsilon/2)\norm{y})^2 - \log(
%   \abs{S(y)} ) } \\
& \leq   (2\uppi)^{-d/2}\exp \defEns{-(\delta^2/8) \norm{y}^2 - \log(
  \abs{S(y) } ) } \\
& \leq   (2\uppi)^{-d/2}\exp \defEns{-(\delta^2/8) \norm{x}^2 - d \log(\epsilon (1+ \delta\epsilon/2)^{-1} ) } \eqsp.
  \end{align*}
  Using this inequality and \eqref{eq:assum_theo_non_geo2} imply $\lim_{\norm{x} \to
    \plusinfty} \inf_{y \in B(x)} \abs{S(x)}q(y,x) =0$ and then
  \eqref{eq:ratio_q_zeros}.} Therefore there exists $R_q \geq 0$ such that for all $x \in
  \rset^d$, $\norm{x} \geq R_q$
  \begin{equation}
\label{eq:def_Rq}
\inf_{y \in B(x)} \frac{q(y,x)}{q(x,y)}  \leq \eta/4 \eqsp.
    \end{equation}
    Now we are able to build the sequence $\{ x_n , n \in \nset\}$ such that for all $n
    \in \nset$, $\norm{x_{n+1}} \geq \max( R_\epsilon, R_q)$ and $\lim_{n \to \plusinfty} \pi(x_n) =
    \plusinfty$. Indeed let $x_0 \in \rset^d$ such that $\norm{x_0} \geq \max( R_\epsilon,
    R_q)$. Assume, we have built the sequence up to the $n$th term and such that for all
    $k=0, \dots, n-1$, $\norm{x_{k+1}} \geq \max( R_\epsilon, R_q)$ and $\pi(x_{k+1}) \geq
    (3/2) \pi(x_k)$. Now we choose $x_{n+1}$ depending
    on $x_n$, satisfying $\pi(x_{n+1}) \geq (3/2) \pi(x_n)$ and $ \norm{x_{n+1}} \geq \max( R_\epsilon, R_q)$. Since
    $\norm{x_n} \geq  \max( R_\epsilon, R_q)$, by
    \eqref{eq:bound_rejection_proba}-\eqref{eq:def_M_non_geo} and \eqref{eq:def_Rq}
  \begin{align*}
\eta &\leq \int_{\rset^d} \alpha(x_n,y) q(x_n,y) \rmd y  \leq \eta/2 + \int_{B(x_n)}
\min \left(1, \frac{\pi(y)q(y,x_n)}{\pi(x_n) q(x_n,y)} \right)  q(x_n,y) \rmd y \\
& \leq \eta/2 + ( \eta/4)\int_{B(x_n)}\frac{\pi(y)}{\pi(x_n)} q(x_n,y) \rmd y \eqsp.
    \end{align*}
    This inequality implies that $\int_{B(x_n)}\frac{\pi(y)}{\pi(x_n)} q(x_n,y) \rmd y  \geq
    2$ and therefore there exists $x_{n+1} \in B(x_n)$ such that $\pi(x_{n+1})
    \geq (3/2)\pi(x_n)$, and since $x_{n+1} \in B(x_n)$ by \eqref{eq:norm_propo_greater},
    $\norm{x_{n+1}} \geq  \max( R_\epsilon, R_q)$. Therefore, we have a sequence $\{x_n ,
    n \in \nset \}$ such that for all $n \in \nset$, $ \pi(x_{n+1}) \geq (3/2)\pi(x_n)$. Since
    by assumption $\pi(x_0) >0$, we get $\lim_{n \to \plusinfty} \pi(x_n) = \plusinfty$,
    which contradicts the assumption that $\pi$ is bounded.
  %\end{proof}
This concludes the proof  of Theorem~\ref{theo:non_geo_erg_Gaussian_MH}.\qed


%\subsection{Technical results}
%\begin{lemma}
%\label{lem:fun_positive}
%The following functions on $\rset^*$ can be extended to continuous and positive functions on $\rset$:
%\begin{enumerate}[(a)]
%\item
%\label{lem:fun_positive_1}
%$\Psi_1 : t \mapsto \{ \rme^{t}-1 - (1/3)t^2 \}/t $.
%\item\label{lem:fun_positive_2}
%$\Psi_2 : t \mapsto \{\rme^{t}-1 + (1/3)(\rme^{-t^2}-1)\}/t $.
%\end{enumerate}
%\end{lemma}
%
%\begin{proof}
%It is straightforward that $\Psi_1$ and $\Psi_2$ can be extended to a continuous function,
%setting $\Psi_1(0) = 1$ and $\Psi_2(0)=1$. Moreover, since for all $t <0$, $\rme^{t} < 1$,
%these two functions are positive on $\rset^*_-$. Now, we study the sign of each one on
%$\rset^*_+$.
%For all $u >0$, $\rme^{u} \geq u $. Integrating this inequality from $0$ to $t >0$, we
%have $\rme^{t} -1 \geq (1/2) t^2$, which implies that $\Psi_1$ is positive on
%$\rset^*_+$. This latter relation also implies that $\Psi_2$ is positive on $\rset^*_+$
%since for all $t >0$, $t \in \rset$, $1-\rme^{t^2} \leq t^2$.
%\end{proof}
%
%\begin{lemma}
%\label{lem:fun_positive_ergodicity1}
%The function $\Psi$ defined on $\coint{3, \plusinfty}$ by
%\begin{multline*}
%\Psi(t) =   1-\defSet{1-\frac{5}{3(t-1)}}^t  \\ - (3/8)t(t-1) \defSet{
%1-\bracket{1-\frac{5}{3(t-1)}}^2 }^2 \defSet{1-\frac{5}{3(t-1)} }^{t-2} \eqsp,
%\end{multline*}
%is positive on $\coint{3, \plusinfty}$.
%\end{lemma}
%
%\begin{proof}
%First  we can write
%\[
%\Psi(t) = 1-\defSet{1-\frac{5}{3(t-1)}}^t   - \frac{25t}{24(t-1)} \defSet{
%2-\frac{5}{3(t-1)} }^2 \defSet{1-\frac{5}{3(t-1)} }^{t-2} \eqsp.
%\]
%Since the functions
%\begin{equation*}
% t \mapsto \defSet{1-\frac{5}{3(t-1)}}^t \eqsp, \quad
% t \mapsto \frac{25t}{24(t-1)} \defSet{
%2-\frac{5}{3(t-1)} }^2 \defSet{1-\frac{5}{3(t-1)} }^{t-2}
%\end{equation*}
%are increasing on $\coint{3,\plusinfty}$, we can conclude that
%\[
%\inf_{ t \in \coint{5, \plusinfty} }\Psi(t) \geq \lim_{ t \to \plusinfty} \Psi(t) = 1- \frac{31 \rme^{-5/3}}{6} >0 \eqsp.
%\]
%\end{proof}
%
%\begin{lemma}
%\label{lem:fun_positive_ergodicity2}
%For all $t,h,\lambda >0$, define the functions $\varrho$, $\varsigma$ and $\Xi$ by:
%\begin{align*}
%\varrho(t) &= (\rme^{-t} - 1) + (2/3)(\rme^{-t^2}- 1) \eqsp, \\
%\varsigma(t) &= (\rme^{-2 t}-1) +(1/3)(\rme^{-4 t^2}-1)  \eqsp, \\
%\Xi(h, \lambda)  &= \lambda \bracket{ 1 - (\varrho(h \lambda)+1)^2  +
%  \varsigma(h \lambda)^{-1}\bracket{4\varrho(h \lambda)^2 + 4 \varrho(h \lambda)^3 +
%    \varrho(h \lambda)^4} }\eqsp.
%\end{align*}
%Then for all $h,\lambda >0$, $\Xi(h, \lambda) >0$.
%\end{lemma}
%
%\begin{proof}
%We just need to check that the function $\psi$ defined by for all $t >0$
%\[
%\psi(t) = 1 - (\varrho(t)+1)^2  +
%  \varsigma(t)^{-1}\bracket{4\varrho(t)^2 + 4 \varrho(t)^3 +
%    \varrho(t)^4} \eqsp,
%\]
%is positive on $\rset_+^*$. But since for all $t >0$, $\varsigma(t) > \varrho(t) +\varrho(t)^2/2$,
%\[
%\psi(t) > 1 - (\varrho(t)+1)^2  +
%  (\varrho(t) +\varrho(t)^2/2)^{-1}\bracket{4\varrho(t)^2 + 4 \varrho(t)^3 +
%    \varrho(t)^4} =0 \eqsp.
%\]
%This concludes the proof.
%\end{proof}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "MCMC_final1"
%%% End: 

